Respect the model: Fine-grained and Robust Explanation with Sharing Ratio Decomposition

The truthfulness of existing explanation methods in authentically elucidating the underlying model's decision-making process has been questioned. Existing methods have deviated from faithfully representing the model, thus susceptible to adversarial attacks. To address this, we propose a novel eXplainable AI (XAI) method called SRD (Sharing Ratio Decomposition), which sincerely reflects the model's inference process, resulting in significantly enhanced robustness in our explanations. Different from the conventional emphasis on the neuronal level, we adopt a vector perspective to consider the intricate nonlinear interactions between filters. We also introduce an interesting observation termed Activation-Pattern-Only Prediction (APOP), letting us emphasize the importance of inactive neurons and redefine relevance encapsulating all relevant information including both active and inactive neurons. Our method, SRD, allows for the recursive decomposition of a Pointwise Feature Vector (PFV), providing a high-resolution Effective Receptive Field (ERF) at any layer.

==> tables/input_scale.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\begin{tabular}{@{}cclccccccclccccccc@{}}
\toprule
                                                  &                               &  & \multicolumn{7}{c}{VGG16}                                                                                      &  & \multicolumn{7}{c}{Resnet50}                                                                                   \\ \midrule
\multicolumn{1}{c|}{}                             &                               &  & Poi.↑         & Att.↑         & Com.↓          & Spa.↑         & Fai.↑         & Lip.↓         & Sen.↓         &  & Poi.↑         & Att.↑         & Com.↓          & Spa.↑         & Fai.↑         & Lip.↓         & Sen.↓         \\ \cmidrule(r){1-2} \cmidrule(lr){4-10} \cmidrule(l){12-18} 
\multicolumn{1}{c|}{\multirow{6}{*}{Input-scale}} & GBP                           &  & {\ul .892}    & {\ul .480}    & {\ul 9.73}     & {\ul .711}    & .022          & {\ul .128}    & {\ul .099}    &  & {\ul .871}    & {\ul .498}    & \textbf{9.62}  & \textbf{.741} & .022          & .156          & .112          \\
\multicolumn{1}{c|}{}                             & InputXGrad                    &  & .781          & .387          & 10.05          & .630          & -.013         & .732          & .181          &  & .639          & .361          & 10.07          & .626          & -.018         & .849          & .178          \\
\multicolumn{1}{c|}{}                             & IG                            &  & .869          & .416          & 10.09          & .618          & -.017         & .463          & .175          &  & .759          & .382          & 10.10          & .614          & -.016         & .688          & .171          \\
\multicolumn{1}{c|}{}                             & Saliency                      &  & .793          & .394          & 10.37          & .494          & .093          & .515          & .181          &  & .654          & .370          & 10.39          & .488          & {\ul .063}    & .587          & .172          \\
\multicolumn{1}{c|}{}                             & LRP\_\{z\textasciicircum{}+\} &  & .855          & .456          & 10.26          & .535          & \textbf{.098} & .583          & .182          &  & .543          & .332          & 9.87           & .572          & .012          & \textbf{.079} & {\ul .105}    \\ \cmidrule(lr){2-2} \cmidrule(lr){4-10} \cmidrule(l){12-18} 
\multicolumn{1}{c|}{}                             & \textbf{SRD(ours)}            &  & \textbf{.925} & \textbf{.561} & \textbf{9.37}  & \textbf{.788} & {\ul .069}    & \textbf{.082} & \textbf{.099} &  & \textbf{.953} & \textbf{.576} & {\ul 9.69}     & {\ul .724}    & \textbf{.082} & {\ul .090}    & \textbf{.104} \\ \cmidrule(r){1-2} \cmidrule(lr){4-10} \cmidrule(l){12-18} 
\multicolumn{1}{c|}{\multirow{5}{*}{High}}        & GradCAM                       &  & .619          & .292          & {\ul 10.27}    & {\ul .537}    & .028          & .273          & .477          &  & .615          & .308          & \textbf{9.62}  & \textbf{.667} & .004          & .654          & .550          \\
\multicolumn{1}{c|}{}                             & GradCAM++                     &  & .662          & .327          & 10.67          & .286          & .045          & .025          & .367          &  & .264          & .268          & 10.73          & .233          & .002          & \textbf{.028} & .658          \\
\multicolumn{1}{c|}{}                             & XGradCAM                      &  & .666          & .314          & 10.43          & .467          & .046          & {\ul .171}    & .384          &  & .610          & .309          & {\ul 9.84}     & .596          & .014          & .552          & .561          \\
\multicolumn{1}{c|}{}                             & LayerCAM                      &  & {\ul .909}    & {\ul .451}    & 10.34          & .507          & {\ul .122}    & .209          & {\ul .219}    &  & {\ul .871}    & {\ul .418}    & 10.48          & .435          & {\ul .096}    & .231          & {\ul .254}    \\ \cmidrule(lr){2-2} \cmidrule(lr){4-10} \cmidrule(l){12-18} 
\multicolumn{1}{c|}{}                             & \textbf{SRD(ours)}            &  & \textbf{.933} & \textbf{.554} & \textbf{9.82}  & \textbf{.696} & \textbf{.123} & \textbf{.126} & \textbf{.205} &  & \textbf{.945} & \textbf{.579} & 9.98           & {\ul .655}    & \textbf{.122} & {\ul .036}    & \textbf{.218} \\ \cmidrule(r){1-2} \cmidrule(lr){4-10} \cmidrule(l){12-18} 
\multicolumn{1}{l|}{\multirow{5}{*}{Middle}}      & GradCAM                       &  & .200          & .216          & \textbf{9.91}  & \textbf{.663} & .013          & .229          & \textbf{.379} &  & .619          & .291          & 10.27          & .513          & .033          & .303          & .672          \\
\multicolumn{1}{l|}{}                             & GradCAM++                     &  & .442          & .302          & 10.74          & .208          & .101          & \textbf{.052} & .570          &  & .597          & .295          & 10.81          & .0874         & .088          & \textbf{.026} & .744          \\
\multicolumn{1}{l|}{}                             & XGradCAM                      &  & .507          & .289          & 10.46          & .452          & .076          & .134          & .467          &  & .716          & .315          & {\ul 10.17}    & {\ul .574}    & .052          & .263          & {\ul .562}    \\
\multicolumn{1}{l|}{}                             & LayerCAM                      &  & {\ul .865}    & {\ul .435}    & 10.52          & .401          & {\ul .199}    & .092          & .423          &  & {\ul .949}    & {\ul .428}    & 10.61          & .339          & {\ul .152}    & .075          & .583          \\ \cmidrule(lr){2-2} \cmidrule(lr){4-10} \cmidrule(l){12-18} 
\multicolumn{1}{l|}{}                             & \textbf{SRD(ours)}            &  & \textbf{.948} & \textbf{.566} & {\ul 10.03}    & {\ul .629}    & \textbf{.206} & {\ul .075}    & {\ul .406}    &  & \textbf{.960} & \textbf{.584} & \textbf{10.06} & \textbf{.630} & \textbf{.154} & {\ul .035}    & \textbf{.505} \\ \cmidrule(r){1-2} \cmidrule(lr){4-10} \cmidrule(l){12-18} 
\multicolumn{1}{l|}{\multirow{5}{*}{Low}}         & GradCAM                       &  & \textbf{.945} & \textbf{.431} & \textbf{10.42} & \textbf{.466} & .175          & {\ul .069}    & .583          &  & \textbf{.946} & .424          & 10.51          & {\ul .411}    & .128          & .024          & .757          \\
\multicolumn{1}{l|}{}                             & GradCAM++                     &  & {\ul .932}    & {\ul .429}    & 10.54          & .351          & .176          & \textbf{.034} & {\ul .570}    &  & {\ul .945}    & .414          & 10.55          & .386          & {\ul .129}    & {\ul .017}    & {\ul .732}    \\
\multicolumn{1}{l|}{}                             & XGradCAM                      &  & .896          & .406          & {\ul 10.45}    & {\ul .446}    & \textbf{.181} & .070          & .576          &  & \textbf{.946} & {\ul .424}    & {\ul 10.51}    & {\ul .411}    & .126          & .024          & .753          \\
\multicolumn{1}{l|}{}                             & LayerCAM                      &  & .869          & .425          & 10.46          & .446          & .175          & .113          & \textbf{.450} &  & .934          & .411          & 10.56          & .379          & .128          & \textbf{.017} & .734          \\
\multicolumn{1}{l|}{}                             & \textbf{SRD(ours)}            &  & \textbf{.945} & .424          & 10.47          & .437          & {\ul .179}    & .072          & .595          &  & \textbf{.946} & \textbf{.544} & \textbf{9.91}  & \textbf{.682} & \textbf{.130} & .041          & \textbf{.600} \\ \bottomrule
\end{tabular}
\end{table}
